MultiK: A Framework for Orchestrating Multiple Specialized Kernels

We present, MultiK, a Linux-based framework 1 that reduces the attack surface for operating system kernels by reducing code bloat. MultiK "orchestrates" multiple kernels that are specialized for individual applications in a transparent manner. This framework is flexible to accommodate different kernel code reduction techniques and, most importantly, run the specialized kernels with near-zero additional runtime overheads. MultiK avoids the overheads of virtualization and runs natively on the system. For instance, an Apache instance is shown to run on a kernel that has (a) 93.68% of its code reduced, (b) 19 of 23 known kernel vulnerabilities eliminated and (c) with negligible performance overheads (0.19%). MultiK is a framework that can integrate with existing code reduction and OS security techniques. We demonstrate this by using D-KUT and S-KUT -- two methods to profile and eliminate unwanted kernel code. The whole process is transparent to the user applications because MultiK does not require a recompilation of the application.

==> code/fmt.tex <==

\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother



==> sections/motivation.tex <==
\section{Motivation}
\label{s:motivation}

In a production setting, the go-to method for a developer to deploy
an application is to install a minimal configuration provided by
a standard distribution out of the box like a minimal-ubuntu-server.
This configuration produces a kernel which is 22MB large. \AU{Would it be misleading that readers think that this is the baseline of our reduction. However, it kernel text only.}
%
Let us consider a popular application stack, e.g a LAMP stack,
which consists of Linux, Apache2, MySQL and a PHP application.
%
From our observations (see \autoref{tab:reduction}) we see that for any given application
on an average only about 800\KB(~10\%) of the entire kernel code is actually used.
%
Effectively the remaining $90\%$ of the kernel is contributing to the attack surface without providing any functional benefit.
%

We can reduce this attack surface by specializing the kernel
for all applications together on a single kernel.
%
But what we see is, orthogonal applications (\eg~Apache2 and ImageMagick)
share only about $20\%$ of the kernel and similar applications
(\eg~Apache2, nginx) up to $80\%$, thus still leaving kernel code
exposed to attacks. To completely eliminate this unused kernel attack surface,
we need a very precise cut.

%

One major problem with achieving this precise cut is lack of
test coverage to completely map out all code paths of the application.
%
This would result in cutting out parts in the kernel which
might be required by the application.
%
And when the application sends a request to kernel that
requires the removed part at runtime,
the customized kernel would fail to serve the request
and thereby, the application fail.
%
Because of this challenge in trade off between
availability and security,
existing approaches are customize kernels with
some level of overestimation.

Kurmus et al. \cite{kurmus} by using a configuration level
granularity include all features related to a certain configuration.
Thus for a LAMP stack they get a reduction of 87\%.
%
KASR uses a page level granularity. It make an entire page of
instruction in memory available to the application available
thus exposing vulnerable areas near execution code paths.
%
Unikernels\cite{unikernels} also overestimates the kernel
to serve the entire system, not just the application.
%
Such effect of overestimation is heightened when
running larger applications. Which is a very typical case with
applications such as web serve, database, language interpreter, etc.

With \sys we are able to get a very precise cut using a basic block level
cut described in \autoref{s:kern-speci}. As well as
maintain stability using a multiplexing framework on top of a base kernel
described in \autoref{s:multik}



==> sections/scenario.tex <==
% explain management and interrupts
\subsection{Scenario}
In this section, we describe scenarios of voluntary/involuntary context
switches, network packet arrivals, and system calls.

% \hl{I'm not clear where we shall put this?}
% We classify events which cause process rescheduling into two categories:
% \begin{itemize}
% \item \textbf{Top-down} events come from the processes. For example, a process issues a \textit{yield()} system call and cause rescheduling directly. Another example is that a process issues an I/O system call and sleeps in order to wait for the I/O operations.
% \item \textbf{Bottom-up} events are triggered by external events. For example, a timer interrupts comes when a process is running. Interrupt handlers have the higher priority so the CPU will immediately executes the timer handler and potentially reschedule processes.
% \end{itemize}
\begin{itemize}
	\item \textbf{Voluntary context switch} \autoref{fig:sc1a} shows how the framework works when a
	      process gives up the CPU voluntarily by issuing either \textit{yield()} or I/O related system calls.

	\item \textbf{Involuntary context switch} \autoref{fig:irq} shows how context switch happens
	      due to the hardware timer event. During the time when \kernelzero is working on the softirq job, \kernelzero
	      picks the next process, for example B, to run from the shared run queue in kernel data. \kernelzero replaces the related
	      register values and switch to switch process B. KernelB is active at this point to that process B can continue.

	\item \textbf{Network packet} \autoref{fig:irq} also shows how \sys responds to network events.
	      After \kernelzero finish the softirq job, kernelA is able to see the processed packet because the kernel data is shared.

	\item \textbf{System call} \autoref{fig:sc3} shows how system calls which do not affect scheduling decisions are handled.

\end{itemize}

\if 0
	\begin{figure}
		\includegraphics[width=\columnwidth,keepaspectratio]{figures-gs/scenario-ctx1}
		\caption{\textbf{Voluntary context switch.} Process A calls a system call,  \textit{yield()}.
			Process A traps into kernelA.
			KernelA picks the next process , B, to run from the shared run queue in kernel
			data. KernelA replaces the related register values in order to switch to
			process B. It is worth mentioning that kernelB is active at this point because
			the CPU is now using the page table from process B. Process B can continue.
		}
		\label{fig:sc1a}
	\end{figure}

	\begin{figure}
		\includegraphics[width=\columnwidth,
			keepaspectratio]{figures-gs/scenario-irq}
		\caption{\textbf{Hardware event handling.} When a hardware event arrives at the time kernelA is executing, it interrupts the CPU and the CPU will jump to the interrupt handler, hardirq. The interrupt handler will place a bottom-half job, softirq, to complete the interrupt handling. Upon exiting the hardirq, the current executing kernel will wake up the softirq worker and switch to \kernelzero. The worker will complete the job and finish the interrupt handling.}
		\label{fig:irq}
	\end{figure}
\fi

% \subsubsection{Network Packet}
% \begin{figure}
% 	\includegraphics[width=\columnwidth, keepaspectratio]
% 	{figures-gs/scenario-irq
% 	\caption{\textbf{Network packet handling.} A network packet which will goes to process A arrives
% when process A is running on kernelA. The Network Interface Controller(NIC)
% triggers a corresponding interrupt to the CPU. The top-half of the interrupt
% handler is executed on the current context, kernelA. This top-half handler
% places a job of the bottom-half interrupt handler. At the time the corresponding
% kernel thread is waken up, it will process the networking packet. Once process A
% is scheduled to run again, kernelA is able to see the packet processed by
% \kernelzero so that process A can continue.}
% 	\label{fig:sc2}
% \end{figure}

\if 0
	\begin{figure}
		\centering \includegraphics[width=0.6\columnwidth, keepaspectratio]
		{figures-gs/scenario-syscall}
		\caption{\textbf{System call.} Process A issues a system call that does not affect
			scheduling, e.g. \textit{open()}. Process A traps into kernelA. KernelA executes the
			procedure for system call \textit{open()} and returns to process A. The execution stays in
			kernelA all the time because there is no context switch.}
		\label{fig:sc3}
	\end{figure}
\fi


==> tbl/perfeval.tex <==
\begin{tabularx}{\textwidth}{lccccc}
	\toprule
	                             & Apache(S/B) & gzip(S/B)   & Redis(S/B)  & STREAM(S/B) \\
	\midrule
	\% of Masked Kernel Text     & 79.01/87.74 & 82.96/90.03 & 78.43/87.61 & 83.24/90.16 \\
	\% of Eliminated ROP Gadgets & 56.81/64.02 & 59.53/65.63 & 56.46/63.88 & 59.75/65.72 \\
	\% of Masked Kernel Symbols  & 80.05/97.74 & 82.62/97.78 & 79.92/97.72 & 82.85/97.78 \\
	\bottomrule
\end{tabularx}

